Approaching Globally Optimal Energy Efficiency in Interference Networks via Machine Learning

This work presents a machine learning approach to optimize the energy efficiency (EE) in a multi-cell wireless network. This optimization problem is non-convex and its global optimum is difficult to find. In the literature, either simple but suboptimal approaches or optimal methods with high complexity and poor scalability are proposed. In contrast, we propose a machine learning framework to approach the global optimum. While the neural network (NN) training takes moderate time, application with the trained model requires very low computational complexity. In particular, we introduce a novel objective function based on stochastic actions to solve the non-convex optimization problem. Besides, we design a dedicated NN architecture for the multi-cell network optimization problems that is permutation-equivariant. It classifies channels according to their roles in the EE computation. In this way, we encode our domain knowledge into the NN design and shed light into the black box of machine learning. Training and testing results show that the proposed method without supervision and with reasonable computational effort achieves an EE close to the global optimum found by the branch-and-bound algorithm. Hence, the proposed approach balances between computational complexity and performance.

==> coverletter.tex <==
Dear editor,

Please find attached our manuscript "Approaching global optimum of energy efficiency in cellular networks via machine learning", which we would like to submit for publication as an original research article in IEEE Transactions on Wireless Communications. Our main contributions are 1) an innovative objective function for non-convex optimization problems based on stochastic action and reparametrization trick, 2) a new neural network architecture, which takes the domain knowledge of wireless communication into account and is permutation-equivariant (i.e., the permutation of user-base station pairs leads to the same permutation of transmit powers automatically).

This work is based on our paper "Non-convex optimization of energy efficient power control in cellular networks via machine learning" with no more than 30% overlap.
The corresponding author is Bile Peng (peng@ifn.ing.tu-bs.de).
We are looking forward to hearing from you.

Sincerely,

Bile Peng, Karl-Ludwig Besser, Ramprasad Raghunath, Eduard Jorswieck



